Grammar compression with probabilistic context-free grammar

We propose a new approach for universal lossless text compression, based on grammar compression. In the literature, a target string $T$ has been compressed as a context-free grammar $G$ in Chomsky normal form satisfying $L(G) = \{T\}$. Such a grammar is often called a \emph{straight-line program} (SLP). In this paper, we consider a probabilistic grammar $G$ that generates $T$, but not necessarily as a unique element of $L(G)$. In order to recover the original text $T$ unambiguously, we keep both the grammar $G$ and the derivation tree of $T$ from the start symbol in $G$, in compressed form. We show some simple evidence that our proposal is indeed more efficient than SLPs for certain texts, both from theoretical and practical points of view.

==> encoding.tex <==
An applied rule sequence has visible redundancy because 
we only need to know which production rule we use when we expand the nondeterministic symbols 
which there are some production rules whose left member is.
For example, in ${ARS}_T$, we don't have to hold production rule which left member is not $v_6$ or $v_9$,
so we can convert (\ref{original_applied_rule_sequence}) to more compact representation ${CARS}_T$ as follows:
\begin{equation}
    \label{compressed_applied_rule_sequence}
    {CARS}_T=r_{10}r_6r_{10}r_7r_{11}
\end{equation}
We can reconstruct an original text with ${PG}_T$ and ${CARS}_T$ because 
we can understand the production rule must be chosen by reading ${CARS}_T$.

In addition, we can encode production rules in ${CARS}_T$ by grouping the production rules whose left member is the same nonterminal symbols 
and arranging them.
For instance, in $v_6$, we assign the code 0 to $r_6$ and the code 1 to $r_7$, and 
in $v_9$, we assign the code 0 to $r_{10}$ and the code 1 to $r_{11}$.
Then we can convert (\ref{compressed_applied_rule_sequence}) to ${ECARS}_T$ as follows:
\begin{equation}
    \label{encoded_applied_rule_sequence}
    {ECARS}_T=00011
\end{equation}
(\ref{encoded_applied_rule_sequence}) is a integer number sequence and they can be encoded easily.
The alphabet size of ${ECARS}_T$ is maximum size of the set of production rule whose elements have the same nonterminal symbols in left side.
If we assign the code to each production rules in the order of increasing (or decreasing) a frequency in use,
the frequency of each code can be unbalanced, so we can use a variety of entropy encoding methods.
Hence, there is a possibility that our framework for grammar compression can achieve a better compression ratio than the methods of existing grammar compression framework 
if the frequency of each production rule is biased.

==> idea.tex <==
Our main idea for new framework of grammar compression is using probabilistic context free grammar {\it{PG}} without some restrictions.
In existing grammar compression methods, we must use the restricted CFG {\it{G}} whose properties are following:
\begin{itemize}
    \item For each nonterminal symbols $A \in V$, there is exactly one production rule in {\it{R}} whose left member is {\it{A}}.
    \item There is no production rule which hold the same nonterminal symbol in both sides.
\end{itemize}
The above properties must be held in CFG used for grammar compression because 
we cannot choose the unique production rules when CFG derives exactly one text in $\Sigma^*$.
In other words, instead of using restricted CFG which can derive exactly one text, 
we can use PCFG {\it{PG}} whose properties are following:
\begin{itemize}
    \item For each nonterminal symbols $A \in V$, there are one or more production rules in {\it{R}} whose left member is {\it{A}}.
    \item For each nonterminal symbols $A \in V$, they can derive some text $w \in \Sigma^*$, that is $A \overset{*}{\Rightarrow} w$.
\end{itemize}
For instance, ${PG}_T$ can be used in our grammar compression framework.
In ${PG}_T$, nonterminal symbols $v_6$ and $v_9$ appears twice in left side of production rules, and 
production rule $v_9 \rightarrow v_8v_9$ holds the same nonterminal symbol $v_9$ in both sides.
All nonterminal symbols $A \in V$ can derive some text 
because nonterminal symbols $v_1$, $v_2$, $v_3$, $v_4$, $v_5$, $v_7$ can obviously derive some text, 
$v_6$ can derive the substring {\it{ab}} or {\it{zb}} and $v_8$ can derive {\it{abcd}} or {\it{zbcd}}, 
and $v_9$ can derive $v_8v_8 \ldots v_8z$.

Due to using PCFG in grammar compression, we introduce new concepts {\it{applied rule sequence}}.
An element $ARS=r_1 \ldots r_m$ of $R^*$ is an applied rule sequence, where $|ARS|=m$ denotes its length.
$r_1,r_2, \ldots ,r_m$ is arranged in the order they are used in the leftmost or rightmost derivation.
It doesn't matter the type of derivation order, but in this paper, we use the leftmost derivation order.
We show the example of an applied rule sequence ${ARS}_T$ with the data string $T=abcdzbcdz$ and ${PG}_T$
We can obtain the text {\it{T}} in following process:
\begin{eqnarray}
    \label{derivation_process}
    S &\Rightarrow& v_9 \Rightarrow v_8v_9 \Rightarrow v_6v_7v_9 \Rightarrow v_1v_2v_7v_9 \Rightarrow av_2v_7v_9 \Rightarrow abv_7v_9 \nonumber \\
    &\Rightarrow& abv_3v_4v_9 \Rightarrow abcv_4v_9 \Rightarrow abcdv_9 \Rightarrow abcdv_8v_9 \nonumber \\
    &\Rightarrow& abcdv_6v_7v_9 \Rightarrow abcdv_5v_2v_7v_9 \Rightarrow abcdzv_2v_7v_9 \\
    &\Rightarrow& abcdzbv_7v_9 \Rightarrow abcdzbv_3v_4v_9 \Rightarrow abcdzbcv_4v_9 \nonumber \\
    &\Rightarrow& abcdzbcdv_9 \Rightarrow abcdzbcdz \nonumber
\end{eqnarray}
From (\ref{derivation_process}), we obtain the applied rule sequence as follows:
\begin{equation}
    \label{original_applied_rule_sequence}
    {ARS}_T=r_{12}r_{10}r_9r_6r_1r_2r_7\\r_3r_4r_{10}r_9r_7r_5r_2r_7r_3r_4r_{11}
\end{equation}
We can reconstruct original text {\it{T}} from ${PG}_T$ and ${ARS}_T$ 
because we can understand which production rule should be applied at the derivation phase.

From the above, our grammar compression framework is defined as follows.
\begin{definition}
    Our grammar compression framework consists of {\it{grammar constructor}}, {\it{rule sequence constructor}},
    {\it{grammar encoder}}, {\it{rule sequence encoder}}, {\it{grammar decoder}}, {\it{rule sequence decoder}}.
    \begin{itemize}
        \item Given a text {\it{T}}, the grammar constructor constructs PCFG ${PG}_T$ such that $T \in L({PG}_T)$, and rule sequence constructor constructs applied rule sequence ${ARS}_T$.
        \item The grammar encoder assigns to ${PG}_T$ a binary codeword which is denoted $B({PG}_T)$.
        \item The rule sequence encoder assigns to ${ARS}_T$ a binary codeword which is denoted $B({ARS}_T)$.
        \item When the grammar and the rule sequence decoder is presented with the codeword $B({PG}_T)$ and $B({ARS}_T)$, the data string {\it{T}} is recovered by first reconstructing the PCFG ${PG}_T$ and the applied rule sequence ${ARS}_T$, and then inferring {\it{T}} from the production rules of ${PG}_T$ and ${ARS}_T$.
    \end{itemize}
\end{definition}

We obviously understand that we only need to hold CFG which can be obtained by excluding the set of probabilities on production rules 
and an applied rule sequence.
However, we can use these probabilities when we encode an applied rule sequence if we can calculate these probabilities properly.
In the next section, we describe this.
